Using sequential drift detection to test the API economy

The API economy refers to the widespread integration of API (advanced programming interface) microservices, where software applications can communicate with each other, as a crucial element in business models and functions. The number of possible ways in which such a system could be used is huge. It is thus desirable to monitor the usage patterns and identify when the system is used in a way that was never used before. This provides a warning to the system analysts and they can ensure uninterrupted operation of the system. In this work we analyze both histograms and call graph of API usage to determine if the usage patterns of the system has shifted. We compare the application of nonparametric statistical and Bayesian sequential analysis to the problem. This is done in a way that overcomes the issue of repeated statistical tests and insures statistical significance of the alerts. The technique was simulated and tested and proven effective in detecting the drift in various scenarios. We also mention modifications to the technique to decrease its memory so that it can respond more quickly when the distribution drift occurs at a delay from when monitoring begins.

==> drift_detection.tex <==
\section{Drift Generation Algorithm}
\label{sec:drift_generation}

Let us consider a test $t$ and $W$ different time windows each associated with a histogram of API calls. Let $H_w^t$ be the histogram associated with window $w$ of test $t$. This histogram can be created using the API logs\footnote{{\bf how to decide window length?}}. So we have
\begin{itemize}
    \item $H_1^t=[h_{11}^t,h_{12}^t,\ldots,h_{1N}^t]$
    \item $H_2^t=[h_{21}^t,h_{22}^t,\ldots,h_{2N}^t]$
    \vdots
    \item $H_W^t =[h_{W1}^t,h_{W2}^T,\ldots,h_{WN}^t]$
\end{itemize}
where $N$ is the number possible API's call.   

We first normalize the histograms. Let the normalized histogram be given by $\hat{H}_w^t$ with 
\begin{eqnarray}
\hat{H}_w^t & = & [\hat{h}_{w1}^t,\hat{h}_{w2}^t,\ldots,\hat{h}_{wN}^t],
\mbox{where,}\\
\hat{h}_{wn}^t & = & \frac{h_{wn}^t}{\sum_{m=1}^N h_{wm}^t}.
\end{eqnarray}

The algorithm describe below identify drift in the observed histogram and helps trigger a new testing effort due to the change of usage pattern in a timely manner\footnote{Add description of detection algorithm.}.   For simplicity we first assume that the set of API does not change but their parameters, parameters semantic and usage may change.   

We next extend this to identify drift over parameters of the API, sequences explicitly.

\subsection{Drift Simulation}

In this section we describe how we simulate drift.  
{\bf Define drift}\\
In order to simulate drift in API calls, we need three histograms of API calls. The first histogram ($h$) is the API call distribution before the drift starts. The second histogram ($h'$) is the API call distribution after the drift period has completed. Let $t_s$ be the start time of drift and $t_e$ be the end of drift. The period $t_s-t_e$ is the time when the API call distribution gradually moves away from $h$ and closer to $h'$. Before $t_s$, the API call distribution was $h$ and after $t_e$ it is $h'$. Let the API calls at any time $t \in [t_s,t_e]$ be sampled from distribution $\tilde{h}_{p(t)}$
where $p(t)$ is a parameter dependent on $t$. 

Give $h$ and $h'$ we next propose an algorithm to construct $\tilde{h}_{p(t)}$. Given any two existing histograms, $h$ and $h'$, let $P(h,h',p)$ creates a new histogram $\tilde{h}_p$ that is obtained by sampling $p$ percent from $h$ and $1-p$ percent from $h'$. This can be done by first choosing $h$ in probability $p$, and then choosing one of the apis, say api $n$ in $h$ with probability equal to the normalized frequency of api $n$ in $h$. After this add a count of one to $\tilde{h}_p$ entry of $n$. 

{\bf An Example} 
\[
h = (4, 3, 2)~~  \\
h' = (5, 2, 3)~~   \\
p = 1/3  \]

Let $P(h, h', 1/3)$.  To create the new histogram $h''$ follow the following process $k$ times:
\begin{enumerate}
\item Chose $h$ with probability 1/3.   Then select an API from $h$  say api 2 with probability 3/9.  Add a count of 1 to api 2 in $\tilde{h}_p$.
\item Choose $h'$ with probability 2/3.  Then chose, say, api 1 with probability 5/10.   Add a count of 1 to api 1 in $h''$ 
\end{enumerate}

Once the process above is followed $k$ times, normalize the vector $\tilde{h}_p$ to obtain the new histogram. Observe that when $p=0$ $\tilde{h}_p$ has the same distribution as $h$ if $k$ is sufficiently large, whereas when $p=1$, $\tilde{h}_p$ has the same distribution as $h'$.

To simulate a drift continuously increase the probability $p$ from 0 to 1.  

%P(h11, h21, p), p(h12, 22, p), ...p(h15, 25, p)
